Attention-Based Real-Time Defenses for Physical Adversarial Attacks in Vision Applications

Deep neural networks exhibit excellent performance in computer vision tasks, but their vulnerability to real-world adversarial attacks, achieved through physical objects that can corrupt their predictions, raises serious security concerns for their application in safety-critical domains. Existing defense methods focus on single-frame analysis and are characterized by high computational costs that limit their applicability in multi-frame scenarios, where real-time decisions are crucial. To address this problem, this paper proposes an efficient attention-based defense mechanism that exploits adversarial channel-attention to quickly identify and track malicious objects in shallow network layers and mask their adversarial effects in a multi-frame setting. This work advances the state of the art by enhancing existing over-activation techniques for real-world adversarial attacks to make them usable in real-time applications. It also introduces an efficient multi-frame defense framework, validating its efficacy through extensive experiments aimed at evaluating both defense performance and computational cost.

==> sections/method_old.tex <==
\section{Background and Preliminaries}

This section concisely provides background and preliminary concepts for the rest of the paper.
We consider vision models that take as input an image with dimensions \(H \times W\) pixels and \(C\) channels, denoted by \(\mathbf{x} \in \mathbb{R}^{3 \times H \times W}\). The model output, denoted as \(f(\mathbf{x})\), depends on the specific vision task under consideration.

For simplicity, the notation is introduced by referring to a simple feed-forward DNN, with a list of layers $\{L^1, ..., L^{N_L}\}$, where the input is forwarded sequentially. To this end, we use the operational notation \(f^{i \to j}\) to denote the processing flow of features from layer \(L^i\) to layer \(L^j\). The layer index 0 is used to refer to the input of the model. For instance, $f(\mathbf{x})$ is equivalent to $f^{0 \to N_L}(\mathbf{x})$ or $f^{k \to N_L}(f^{0 \to k}(\mathbf{x}))$. %This allows to split the inference process in a intermediate layer. 

%means the complete inference process across all layers, i.e., $f(x)$. Equivalently, \(f^{k \to N_L}(f^{0 \to k}(x))\) generalizes this notation to describe the inference process from an intermediate layer \(k\) to the final layer \(N_L\). 

{\color{red} TODO: introduce here the \emph{activations} of a layer, also defining the corresponding symbol.}
{\color{blue} migliorata definition in 3.2}

\subsection{Real-World Adversarial Attacks}
Real-world adversarial attacks can be generated by introducing \textit{adversarial physical objects} into specific regions of the scene captured by the input image \(\mathbf{x}\). Following previous work, we model these objects as rectangular patches denoted by \(\bm{\delta}\), where \(\bm{\delta}\) is an image of size \(\tilde{H} \times \tilde{W}\) with \(C\) channels, where \(\tilde{H} \leq H\) and \(\tilde{W} \leq W\). Crafting an adversarial patch involves solving an optimization problem aimed at minimizing a specific attack loss function, while enhancing the robustness of the patch features against realistic transformations that can occur while filming the patch in the physical world~\cite{pmlr-v80-athalye18b}.

Formally, we craft an adversarial patch \(\bm{\delta}\) by solving the following optimization problem:
\begin{equation}
    \bm{\delta} = \argmin_{\bm{\delta}}~\mathbb{E}_{\mathbf{x}\sim\mathbf{X}, \gamma\sim\bm{\Gamma}} ~ \mathcal{L}_{\text{Adv}}(f(\tilde{\bm{x}}), \mathbf{y}_{\text{Adv}}),
\label{eq:adv}
\end{equation}


%AB - {\color{red} $\gamma$ dovrebbe essere usata da qualche parte nella formula}
%GR - Ok - dovrei aver sistemato

\noindent where \(\mathbf{X}\) is a set of images to attack, $\tilde{\bm{x}} = \bm{x} + \gamma(\bm{\delta})$ is the attacked image, \(\bm{\Gamma}\) is a set of appearance and placement transformations that can be randomly selected to apply a patch, 
\(\mathbf{y}_{\text{Adv}}\) is the adversarial output target, and \(\mathcal{L}_{\text{Adv}}\) is the adversarial loss function that specifies the objective of the attacker{\color{blue}, the lower \(\mathcal{L}_{\text{Adv}}\)  the more adversarial effect}.
{\color{red} Add here the key property of \(\mathcal{L}_{\text{Adv}}\): the lower the more adversarial effect (right?)}
%For instance, if the objective is to execute an untargeted attack, the adversarial target \(\mathbf{y}_{\text{Adv}}\) can be any but the ground truth \(\mathbf{y}\) and hence a classical cross-entropy loss function $\mathcal{L}$ can be used as \(-\mathcal{L}(f(\tilde{\mathbf{x}}), \mathbf{y})\).
Please refer to \cite{pmlr-v80-athalye18b, brown_adversarial_2018, rossolini_tnnls_2023} for further details.


\subsection{Defense Mechanisms and Internal Analysis}
\label{sec:internal_analysis}
As discussed in Section 2, several defense strategies have been proposed in the literature to mitigate real-world adversarial attacks, particularly in single-frame applications. In this context, our approach aligns closely with works that perform internal analysis of neural models during inference. 

Following this paradigm, we denote by $\bm{h}^{l} \in \mathbb{R}^{C^l \times H^l \times W^l}$ the features produced by any layer $L^l$, where $C^l, H^l, W^l$ are the corresponding tensor dimensions, i.e., $\bm{h}^{l}=f^{0 \to l}(\mathbf{x})$.
Essentially, given an attacked input $\tilde{\mathbf{x}}$, defense mechanisms based on internal analysis analyze one or more deep features to extract a heatmap $\mathcal{H} \in \mathbb{R}^{H^l \times W^l}$ that effectively highlight the position of the patch within the image. Then, the heatmap $\mathcal{H}$ is binarized, using a threshold, to obtain a mask $\mathcal{M_\delta} \in \{0,1\}^{H^l \times W^l}$.
Formally speaking, these steps can be summarized by means of a function $\Lambda^\xi:  \mathbb{R}^{C^l \times H^l \times W^l} \to \{0,1\}^{H^l \times W^l} $, which takes as input the features $\bm{h}^{l}$ from a given layer and produces a mask based on a pre-determined threshold $\xi$.
%Then, the heatmap $\mathcal{H}$ is binarized into a mask $\mathcal{M_\delta} \in \{0,1\}^{H^l \times W^l}$, 
The resulting mask can then be applied at any layer $L^z$ (e.g., even the input image itself, $z=0$) to filter out the adversarial object, thereby aiming at making the attack ineffective, i.e.,
\begin{equation}
    f^{z \to N_L}( f^{0 \to z}(\tilde{\mathbf{x}}) \odot r^{l \to z}(\mathcal{M_\delta})) \approx f(\mathbf{x}),
\end{equation}
where $\odot$ is the Hadamard product operator and $r^{l \to z}$ is a resizing function to apply a mask extracted at the $l$-th layer to the $z$-th layer (clearly not needed when $l=z$). 
In general, function $r^{l \to z}$ consists of a simple interpolation.
%In general, In some cases, a resizing function may need to be applied to the mask whenever the addressed layer refers to a different spatial dimension. This issue is generally addressed by performing a simple interpolation.

Since this work proposes a defense mechanism for multi-frame cases, from Section~\ref{sec:adv_multiple} on we adopt a discrete-time notation with the superscript $k$ to refer to the symbols introduced above when related to the $k$-th frame, where $k \in \{0, \ldots, K\}$.

\section{Adversarial-Channel Attention}
Inspired by prior research on RW attacks and internal over-activation analysis for neural networks, 
we observed that attacks can be detected by even analyzing shallow network layers (as opposed to deep layers as done by previous work).
In the following, we provide insights into the existence of over-activation patterns within shallow layers and then address the definition of \emph{adversarial trace}, which is later used to enable the implementation of an adversarial attention mechanism for multi-frame scenarios.

\subsection{Single-frame Adversarial Attention Analysis}
We start by providing insights that link abnormal activations induced by adversarial objects with a specific pattern of channels in the shallow layers.
%This connection primarily arises from the behavior of trained models, which enforce hierarchical feature relationships in neural networks \cite{zeiler2014visualizing}.
%This connection primarily arises from the nature of trained models, which inherently enforce hierarchical feature relationships in neural networks \cite{zeiler2014visualizing}.

\begin{oss}
An adversarial object $\delta$ is designed to minimize a specific adversarial loss function by influencing certain network features (see Eq.\eqref{eq:adv}). %~\cite{yu2021defending}, \cite{rossolini2023defending}. 
%which are in turn linked to the robustness of the attack against different backgrounds and samples.
%This observation can be formalized as follows.
As for instance shown in Figure \ref{f:sec3}(a), we argue that in any layer $L^l$ with activations $\bm{h}^{l}$, there exists a subset of channels targeted by the adversarial object. The channels can be identified by applying some channel weights $\boldsymbol{\sigma} \in [0,1]^{C^l}$ that, if applied to $\bm{h}^{l}$, amplify the adversarial features, i.e.,
%if the activations $\bm{h}^{l}$ are channel-wise weighted with $\boldsymbol{\sigma}$, the adversarial effect is consistently more pronounced, that is:
\[
\mathcal{L}_{\text{Adv}}(f^{l\to N_L}(\boldsymbol{\sigma} \cdot \bm{h}^l), \mathbf{y}_{\text{Adv}})~ \leq ~\mathcal{L}_{\text{Adv}}(f^{l\to N_L}(\bm{h}^l), \mathbf{y}_{\text{Adv}}).
\]
\end{oss}
%compared to uniform averaging across all channels.
\begin{oss}
As known from previous work~\cite{yu2021defending}, real-world adversarial features are characterized by over-activations.
Therefore, from the perspective of an internal analysis (as introduced in Section \ref{sec:internal_analysis}),
%since a higher adversarial effect is linked to a higher over-activation effect \cite{ yu2021defending, rossolini2023defending, co_real}, 
a proper definition of $\boldsymbol{\sigma}$ also allows focusing on the channels that are more subject to over-activation within the attacked area. This results in a better separation of the attacked area from all the others in the heatmap $\mathcal{H}$. The observation can be formulated in terms of intersection-over-union (IoU) \cite{iou_survey} between the predicted attacked area and the exact one:
\[
\textit{IoU}\left( \Lambda^{\xi^{'}}(\boldsymbol{\sigma} \cdot \bm{h}^l),~\mathcal{M}_{\textit{GT}} \right) \geq \textit{IoU}\left( \Lambda^{\xi^{''}}(\bm{h}^l),~\mathcal{M}_{\textit{GT}} \right),
\]
\noindent
where $\mathcal{M}_{\textit{GT}}$ is the ground truth mask, and $\xi^{'}$ and $\xi^{''}$ are the optimal hypothetical thresholds within the two addressed settings. 
\end{oss}

%$\boldsymbol{\sigma}$ can be represented as channel weights that maximize the separation between the activation in the attacked regions and the one in all other regions. Following the defense approach based on internal analysis, it can be seen as a maximum of the intersection-over-union (IoU) \cite{iou_survey} between the attacked area and the others:
% \begin{equation}
% \max_{\boldsymbol{\sigma}}~~~  \sum_{c, i, j = 1}^{C^l, H^l, W^l} \boldsymbol{\sigma}_c  \left(
% \frac{(\bm{h}^l \odot \mathcal{M}_{\bm{\delta}})_{c,i,j}}{|\mathcal{M}_{\bm{\delta}} |} 
% - 
% \frac{(\bm{h}^l \odot \bar{\mathcal{M}}_{\bm{\delta}})_{c, i,j}}{|\bar{\mathcal{M}}_{\bm{\delta}} |}\right),
% \end{equation}
% \begin{equation}
% \max_{\boldsymbol{\sigma}}~~~  \textit{IoU}~\left( \mathcal{M}_{\bm{\delta}},~\mathcal{M}_{\textit{GT}} \right)
% \end{equation}
%Here, $\mathcal{M}_\bm{\delta}$ represents the ground truth mask of the adversarial object $\bm{\delta}$, and 
% \noindent 
% where $\mathcal{M}_{\bm{\delta}} = \Lambda^\xi(\boldsymbol{\sigma} \cdot \bm{h}^l)$ and $\mathcal{M}_{\textit{GT}}$ are the predicted and exact mask, respectively. 


%the exact position of the patch.
%where $\bar{\mathcal{M}}_{\bm{\delta}} = I - \mathcal{M}_{\bm{\delta}}$ is the area outside the adversarial attack. The first term denotes the average activation within the adversarial area, while the second term represents the average activation in the other areas. In simpler terms, channel attention guided by $\boldsymbol{\sigma}$ helps separate the activation magnitude between the adversarial area and the non-adversarial areas.


Channel weights $\boldsymbol{\sigma}$ play a pivotal role in efficiently 
%While the assumption of specific channels may seem straightforward, it plays a pivotal role in 
identifying over-activated areas associated with adversarial features, even in shallow layers. 
In fact, while the over-activation phenomenon may look straightforward to detect, 
our preliminary experiments revealed that simple operations directly applied to all channels, e.g., a channel-wise sum compared to a threshold, do not allow detecting the presence of adversarial objects.

%This is because, as shown in Figure \ref{f:sec3}(a), only specific channels are targeted by adversarial features so that a simple channel-wise sum of the $\bm{h}^l$ cannot highlight in easily distinguishable manner the presence of adversarial objects. 
%this concept by showing how in a given shallow layer the adversarial attack focuses on specific channels. 

\begin{figure}[ht]
\begin{center}
\includegraphics[width=\columnwidth]{img/im_sec3.pdf}
\caption{\small{(a) Mean channel-wise activation from the first spatial BiSeNet \cite{bisenet_paper} layer during the inference of the attacked image; (b) representation of the heatmap with and without the attention mechanisms.}}
\label{f:sec3}
\end{center}
\end{figure}


\subsection{Adversarial Attention Implementation}
\label{sec:adv_multiple}
Following the above observations, we propose a practical use and definition of channel weights $\boldsymbol{\sigma}$ for consecutive frames. As anticipated in the paper introduction (see Figure~\ref{f:fig_intro}), the proposed implementation is conceived to be complemented with a defense method capable of providing a starting mask $\mathcal{M}^{0}_{\bm{\delta}}$. When and how this starting mask needs to be computed 
will be discussed in Section~\ref{s:ACAT}, where the complete defense framework is presented.

{\color{red}explain the approach at a high level: we compute heatmap, we predict a mask at time k, we compute the weights, etc.}

\begin{definition}[Adversarial Trace]
The adversarial trace is a sequence of weights that, if applied to the activations of a certain layer over time, allows detecting over-activations.
Formally, given a layer $L^l$, the adversarial trace at time $k$, denoted by $\boldsymbol{\sigma}^{k}_{{\bm{\delta}}}$, is a vector of $C^l$ elements in $[0, 1]$.
%, that represent the contribution of each channel in over activating adversarial features in $L^l$ at time $k$. 
The elements of the adversarial trace are computed by leveraging the mask computed at the $k$:
\begin{equation}
\boldsymbol{\sigma}^{k}_{\delta} = \mathcal{N}\left(\frac{\sum_{i,j=1}^{H, W}\left(\bm{h}^{l,k}_{i,j,c} \odot \mathcal{M}^k_{\bm{\delta}}\right)}{|\mathcal{M}^k_{\bm{\delta}}|} - \frac{ \sum_{i,j=1}^{H, W}\left(\bm{h}^{l,k}_{i,j,c} \odot {\bar{\mathcal{M}}^k_{\bm{\delta}}}\right)} {|{\bar{\mathcal{M}}^k_{\bm{\delta}}} |}\right),
\label{eq:adv_trace}
\end{equation}
where $\mathcal{M}^k_{\bm{\delta}}$ is the predicted mask at time $k$, $\bar{\mathcal{M}}^k_{\bm{\delta}}$ denotes a complementary mask to address all other tensor values not interested by $\mathcal{M}^k_{\bm{\delta}}$, and $\mathcal{N}$ represents a normalization function that scales the values to the $[0, 1]$ range. In our configuration, we implement the $\mathcal{N}$ as a ReLU function followed by a channel-wise min-max normalization.

In particular, the first fractional term in Eq.~\eqref{eq:adv_trace} provides attention to over-activated patterns within the area of the adversarial object, while the second term provides negative attention to activations outside the same.
\end{definition}

\paragraph{Leveraging the Adversarial Trace}
The adversarial trace enables the computation of an accurate heatmap $\mathcal{H}^k$ at each time $k$ by leveraging the weights $\boldsymbol{\sigma}^{k-1}_{\delta}$ computed at the previous iteration:
%Since computing the adversarial trace at time $k$ requires knowledge of the predicted mask at that specific time, it is impossible to directly use $\boldsymbol{\sigma}^{k}_{\bm{\delta}}$ to extract $\mathcal{M}^{k}_{\bm{\delta}}$. To overcome this, following an iterative temporal principle, we compute 
%The heatmap $\mathcal{H}^k$ based on the previous activation trace $\boldsymbol{\sigma}^{k-1}_{\delta}$:
\begin{equation}
\mathcal{H}^k = \sum_{c = 1}^{C^l} (\boldsymbol{\bm{\sigma}}^{k-1}_{\bm{\delta}})^{\tau} \cdot \bm{h}^{l,k},
\end{equation}
\noindent where parameter $\tau$ is introduced to amplify the attention pattern within the heatmap. Figure~\ref{f:sec3}(b) shows the benefits of using attention based on the adversarial trace. 

Once the heatmap is obtained a threshold parameter $\xi^k$ can be used to devise the binary mask $\mathcal{M}^{k}_\delta$.

\paragraph{Threshold definition}
Differently from previous work, which adopted a static threshold computed offline on a calibration data set, this work adopts an adaptive threshold that is dynamically computed  frame by frame. This is required because the attention mechanism weights channels dynamically, making it hard to compute a threshold in advance. The threshold is computed as follows: 
\[
\xi^k = \max( \mathcal{\bar{H}}^{k-1} ) + \psi(\mathcal{\bar{H}}^{k-1})
\],
\noindent where $\mathcal{\bar{H}}^{k-1} = \mathcal{H}^{k-1} \odot \mathcal{\bar{M}}^{k-1}_{\bm{\delta}} $ represents the heatmap that pertains solely to non-adversarial features, and $\psi(\mathcal{\bar{H}}^{k-1})$ is an additional margin added to the threshold to reinforce the avoidance of false positive. It consists of the distance from the mean activation value of the non-adversarial features (50th percentile) and a higher percentile (e.g., 70th percentile), this helps add an additional margin not based on outliers in the not-adversarial distribution. 

%AB- arrivato qui

It is worth observing that in our experiments we observed that areas close to the adversarial object can also jeopardize the threshold computation across multiple frames. This is because the over-activation can continuously decrease from attacked pixels to non-attacked pixels. To address this, we employed a dilation function to compute $\mathcal{\bar{H}}^{k-1}$, where the available mask is dilated with an average kernel to introduce an area of uncertainty not considered in the threshold calculation.

%In essence, this threshold is set higher than the maximum value in $\mathcal{\bar{H}}^k$ to avoid false positives, ensuring that non-adversarial objects covered by the masks are not erroneously identified as adversarial.

%MODIFICARE DICENDO CHE LA THRESHOLD VIENE AGGIUSTATA AD OGNI FRAME COME PRIMA E MENZIONARE IL TRUCCO DEL DILATION. 

%We decided not to update the threshold at each frame for conservative reasons. Assuming that the portion of the predicted mask may not cover the entire adversarial area in the subsequent frames, increasing the threshold frame by frame raises the risk of overlooking less adversarial parts in the subsequent frames.


\paragraph{Illustration of the approach.}
We provide a schematic representation of the approach that recaps the update and use of the adversarial trace in Figure 2. In practice, we also introduce a gaussian filter for the heatmap computation, which was omitted in the previous analysis for simplicity. As highlighted by related works \cite{rossolini2023defending}, denoising filters help mitigate the effects of small spurious activations.

In summary, the extraction and continuous update of the adversarial trace allows us to dynamically focus on the most crucial channels. In the next section, we provide a detailed description of the tracking framework.
%changing contexts and variations in the appearance of adversarial patches.
\begin{figure}[ht]
\begin{center}
\includegraphics[width=\columnwidth]{img/scheme_functions.pdf}
\caption{\small{Operation performed with the run-time trace and update of the adversarial trace. See \ref{alg:algorithm} for more details.{\color{red} sistemare eq number e threshold, mettere trace symbol.}}}
\label{f:pl1}
\end{center}
\end{figure}
% It's worth noting that the update of the threshold and trace can be applied at each frame or after a predefined number of frames. This flexibility, coupled with the approach's heavy reliance on the channel dimension, makes it robust to possible changes and low frame rates, as discussed in our experimental findings.

 
 \section{ACAT framework}\label{s:ACAT}
In this section, we integrate the previously mentioned approach into the processing loop of multi-frame applications. Algorithm \ref{alg:algorithm} outlines the inference pipeline adopted when utilizing the tracking mechanism.

\input{algorithms/alg1}

For each frame, it checks if $\boldsymbol{\sigma}_{\delta}$ exists. If it is not, it means no prior adversarial attack was detected and linked to an ACAT thread. In this case, the algorithm runs a defense method to monitor the current frame $\bm{x}^k$. If $\mathcal{M}_{\delta}$ reports an adversarial attack, i.e., the mask is not 'none', the algorithm initializes an ACAT mechanism by computing the adversarial trace $\bm{\sigma_{\delta}}$ and a threshold $\xi$. Then conclude the iteration by forwarding the cleaned features using the known mask.

Once $\boldsymbol{\sigma}_{\delta}$ is set (indicating an ongoing attack), the algorithm executes the ACAT trace on the current frame $\bm
{x}$, leveraging the previous trace and threshold to compute a new mask. If the mask is still available (line 18, i.e., larger than $\lambda_\mathcal{M}$), it updates the trace and the threshold (line 22 and 23) and filters out the adversarial features, thus forwarding the new activations into the remaining inference part (line 24). 

\paragraph{Stop criterion}
As shown in \textit{line 18} of the algorithm, the stop criterion is utilized to halt the tracking mechanism. Knowing a reasonable connection between the mask size and the induced adversarial effect \cite{rossolini2023defending}, we use the number of pixels detected in the predicted mask  to decide whether to stop tracking or not. Specifically, when the size of the mask is lower than $\lambda_\mathcal{M}$, we assume that the patch is too far or not well detected. Note that users have the flexibility to customize this aspect, allowing the mechanism to remain active but skipping the update part or terminating the tracking process.
In the tested version, once the stop condition succeeds, we terminate the tracking, waiting for a new detection of the attack from a defense mechanism.
%to detect if an attack exists with a defense mechanism. CONTROLLARE QUESTA COSA
%For instance, the object can be overlapped by some object and may reappear after a few frames. In such cases, it is sufficient to remove the initialization of $\delta$ (line 19).

\paragraph{Timing analysis}
In the presence of an adversarial attack, algorithm \ref{alg:algorithm} shows timing benefits with respect to other strategies. Single-frame approaches may involve the use of additional models or the repetition of an entire inference when detecting the presence of the patch (as seen in lines 5 and 10). In contrast, our approach, once activated, incurs an overall computational cost similar to a single inference. 






%#################
% more extensive proof 
\begin{comment}
% W can provide a mathematical formulation to reinforce the observation that in an efficient neural network layer, channels should have distinct patterns or features to be useful. Let's consider a layer \(L\) with \(C^L\) channels. The goal of this layer is to contribute to the final logit \(y_i\) for a specific class \(i\).

% We can express the contribution of each channel \(c \in C^L\) to the final logit \(y_i\) as follows:

% \[y_i = \sum_{c \in C^L} w_{ic} \cdot h_c^L\]

% Here:
% - \(w_{ic}\) represents the weight connecting channel \(c\) to the final logit \(y_i\).
% - \(h_c^L\) represents the activation of channel \(c\) in layer \(L\).

% In an ideal scenario, each weight \(w_{ic}\) should emphasize specific patterns or features captured by the corresponding channel \(c\) that are relevant to class \(i\). This means that \(w_{ic}\) should not be uniform for all \(c\) but should vary according to the importance of the feature or pattern.

% Now, let's consider the extreme case where all channels in layer \(L\) have the same importance for the final logit \(y_i\), meaning \(w_{ic}\) is uniform for all \(c\). We can denote this uniform importance as \(w_i\):

% \[y_i = \sum_{c \in C^L} w_i \cdot h_c^L\]

% In this case, the layer \(L\) is essentially treating all channels equally, which is highly unlikely to be efficient for capturing meaningful patterns or features. It would be challenging for such a layer to differentiate between different input patterns or contribute effectively to the network's ability to discriminate between classes.

% So, mathematically, we can assert that for an efficient neural network layer, \(w_{ic}\) should not be uniform across all channels, and each channel should have distinct patterns or features relevant to its task. Uniform importance of channels would not lead to optimal performance in a deep neural network.
\end{comment}


==> tables/ablation.tex <==
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Step 1} & \textbf{Step 2} & \textbf{Step 3} & \textbf{Step 4} & \textbf{Precision} \\
\hline
\checkmark & & & & 0.89 \\
\hline
\checkmark & \checkmark & & & 0.91 \\
\hline
\checkmark & \checkmark & \checkmark & & 0.94 \\
\hline
\checkmark & \checkmark & \checkmark & \checkmark & 0.97 \\
\hline
\end{tabular}
